Dynamics of Hot QCD Matter 2024 -- Bulk Properties

The second Hot QCD Matter 2024 conference at IIT Mandi focused on various ongoing topics in high-energy heavy-ion collisions, encompassing theoretical and experimental perspectives. This proceedings volume includes 19 contributions that collectively explore diverse aspects of the bulk properties of hot QCD matter. The topics encompass the dynamics of electromagnetic fields, transport properties, hadronic matter, spin hydrodynamics, and the role of conserved charges in high-energy environments. These studies significantly enhance our understanding of the complex dynamics of hot QCD matter, the quark-gluon plasma (QGP) formed in high-energy nuclear collisions. Advances in theoretical frameworks, including hydrodynamics, spin dynamics, and fluctuation studies, aim to improve theoretical calculations and refine our knowledge of the thermodynamic properties of strongly interacting matter. Experimental efforts, such as those conducted by the ALICE and STAR collaborations, play a vital role in validating these theoretical predictions and deepening our insight into the QCD phase diagram, collectivity in small systems, and the early-stage behavior of strongly interacting matter. Combining theoretical models with experimental observations offers a comprehensive understanding of the extreme conditions encountered in relativistic heavy-ion and proton-proton collisions.

==> Lokesh/bib.tex <==
%%%%%%%%Lokesh begins%%%%%%%%

%\cite{STAR:2005gfr}
\bibitem{STAR:2005gfr}
J.~Adams \textit{et al.} [STAR],
%``Experimental and theoretical challenges in the search for the quark gluon plasma: The STAR Collaboration's critical assessment of the evidence from RHIC collisions,''
Nucl. Phys. A \textbf{757}, 102-183 (2005).
%doi:10.1016/j.nuclphysa.2005.03.085
%[arXiv:nucl-ex/0501009 [nucl-ex]].
%3541 citations counted in INSPIRE as of 08 Jul 2022

%\cite{ALICE:2008ngc}
\bibitem{ALICE:2008ngc}
K.~Aamodt \textit{et al.} [ALICE],
%``The ALICE experiment at the CERN LHC,''
JINST \textbf{3}, S08002 (2008).
%doi:10.1088/1748-0221/3/08/S08002
%3300 citations counted in INSPIRE as of 08 Jul 2022


%\cite{Cleymans:2005xv}
\bibitem{Cleymans:2005xv}
J.~Cleymans %H.~Oeschler, K.~Redlich and S.~Wheaton,
%``Comparison of chemical freeze-out criteria in heavy-ion collisions,''
\textit{et al.}, 
Phys.Rev.C \textbf{73}, 034905 (2006).
%doi:10.1103/PhysRevC.73.034905
%[arXiv:hep-ph/0511094 [hep-ph]].
%733 citations counted in INSPIRE as of 23 Oct 2024


\bibitem{qcd_ph}
H. Caines, Nucl. Phys. A 967, 121 (2017).

%\cite{STAR:2017sal}
\bibitem{STAR:2017sal}
L.~Adamczyk \textit{et al.} [STAR],
%``Bulk Properties of the Medium Produced in Relativistic Heavy-Ion Collisions from the Beam Energy Scan Program,''
Phys. Rev. C \textbf{96}, no.4, 044904 (2017).
%doi:10.1103/PhysRevC.96.044904
%[arXiv:1701.07065 [nucl-ex]].
%643 citations counted in INSPIRE as of 23 Oct 2024



%\cite{STAR:2024bpc}
\bibitem{STAR:2024bpc}
STAR Collaboration,
%``Temperature Measurement of Quark-Gluon Plasma at Different Stages,''
[arXiv:2402.01998 [nucl-ex]].
%3 citations counted in INSPIRE as of 23 Oct 2024

%\cite{ALICE:2021mfm}
\bibitem{cp_sqm24}
Y. Zhang (for the STAR Collaboration), Strangeness in Quark Matter (2024).

\bibitem{str_fix_sqm24}
H. Li (for the STAR Collaboration), Strangeness in Quark Matter (2024).

\bibitem{v2_fix_sqm24}
S. Shi (for the STAR Collaboration), Strangeness in Quark Matter (2024).

\bibitem{str_dau_sqm24}
I. Aggarwal (for the STAR Collaboration), Strangeness in Quark Matter (2024).

\bibitem{v2_pp_sqm24}
D. Sarkar (for the ALICE Collaboration), Strangeness in Quark Matter (2024).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%Lokesh ends%%%%%%%%










==> merged-bib.tex <==
%%%%% Anuraag Rathore %%%%%%

\bibitem{Acharya2019}
Acharya S, Adamová D, Adhya SP, et al. Charged-particle production as a function of multiplicity and transverse spherocity in pp collisions at $\sqrt{s} = 5.02$ and 13 TeV. \textit{The European Physical Journal C} 2019; 79:1–22.

\bibitem{Skands2014}
Skands P, Carrazza S, and Rojo J. Tuning PYTHIA 8.1: the Monash 2013 tune. \textit{The European Physical Journal C} 2014; 74:3024.

\bibitem{Acharya2023}
Acharya S, Adamová D, Adler A, et al. Multiplicity dependence of charged-particle production in pp, p–Pb, Xe–Xe, and Pb–Pb collisions at the LHC. \textit{Physics Letters B} 2023; 845:138110.

\bibitem{Ortiz2019}
Ortiz A and Palomo LV. Probing color reconnection with underlying event observables at the LHC energies. \textit{Physical Review D} 2019; 99:034027.

\bibitem{Ortiz2024}
Ortiz A, Valencia Palomo L, and Minjares Neriz VM. Study of Transverse-Spherocity Biased pp Collisions at the LHC Energies Using the PYTHIA 8 Event Generator. \textit{Universe} 2024; 10:30.

\bibitem{Acharya2024}
Acharya S, Adamová D, Aglieri Rinella G, et al. Light-flavor particle production in high-multiplicity pp collisions at $\sqrt{\textrm{s}} = 13$ TeV as a function of transverse spherocity. \textit{Journal of High Energy Physics} 2024; 2024:1–57.

\bibitem{Palni2020}
Palni P, Khuntia A, and Bartalini P. Evolution of strange and multi-strange hadron production with relative transverse multiplicity activity in underlying event. \textit{The European Physical Journal C} 2020; 80:919.



%%%%%%%%%%% Amaresh Jaiswal %%%%%%%%


\bibitem{Niida:2024ntm}
T.~Niida and S.~A.~Voloshin,
%``Polarization phenomenon in heavy-ion collisions,''
Int. J. Mod. Phys. E \textbf{33} (2024) no.09, 2430010
%doi:10.1142/S0218301324300108
[arXiv:2404.11042 [nucl-ex]].
%8 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Florkowski:2018fap}
\bibitem{Florkowski:2018fap}
W.~Florkowski, A.~Kumar and R.~Ryblewski,
%``Relativistic hydrodynamics for spin-polarized fluids,''
Prog. Part. Nucl. Phys. \textbf{108} (2019), 103709
%doi:10.1016/j.ppnp.2019.07.001
[arXiv:1811.04409 [nucl-th]].
%185 citations counted in INSPIRE as of 14 Nov 2024

%\cite{Dey:2023hft}
\bibitem{Dey:2023hft}
S.~Dey, W.~Florkowski, A.~Jaiswal and R.~Ryblewski,
%``Pseudogauge freedom and the SO(3) algebra of spin operators,''
Phys. Lett. B \textbf{843} (2023), 137994
%doi:10.1016/j.physletb.2023.137994
[arXiv:2303.05271 [hep-th]].
%14 citations counted in INSPIRE as of 12 Nov 2024

%\cite{Becattini:2017gcx}
\bibitem{Becattini:2017gcx}
F.~Becattini and I.~Karpenko,
%``Collective Longitudinal Polarization in Relativistic Heavy-Ion Collisions at Very High Energy,''
Phys. Rev. Lett. \textbf{120} (2018) no.1, 012302
%doi:10.1103/PhysRevLett.120.012302
[arXiv:1707.07984 [nucl-th]].
%198 citations counted in INSPIRE as of 14 Nov 2024

%\cite{Banerjee:2024xnd}
\bibitem{Banerjee:2024xnd}
S.~Banerjee, S.~Bhadury, W.~Florkowski, A.~Jaiswal and R.~Ryblewski,
%``Longitudinal spin polarization in a thermal model with dissipative corrections,''
[arXiv:2405.05089 [hep-ph]].
%5 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Hehl:1976vr}
\bibitem{Hehl:1976vr}
F.~W.~Hehl,
%``On the Energy Tensor of Spinning Massive Matter in Classical Field Theory and General Relativity,''
Rept. Math. Phys. \textbf{9} (1976), 55-82.
%doi:10.1016/0034-4877(76)90016-1
%106 citations counted in INSPIRE as of 12 Nov 2024

%\cite{STAR:2019erd}
\bibitem{STAR:2019erd}
J.~Adam \textit{et al.} [STAR],
%``Polarization of $\Lambda$ ($\bar{\Lambda}$) hyperons along the beam direction in Au+Au collisions at $\sqrt{s_{_{NN}}}$ = 200 GeV,''
Phys. Rev. Lett. \textbf{123} (2019) no.13, 132301
%doi:10.1103/PhysRevLett.123.132301
[arXiv:1905.11917 [nucl-ex]].
%236 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Fu:2021pok}
\bibitem{Fu:2021pok}
B.~Fu, S.~Y.~F.~Liu, L.~Pang, H.~Song and Y.~Yin,
%``Shear-Induced Spin Polarization in Heavy-Ion Collisions,''
Phys. Rev. Lett. \textbf{127} (2021) no.14, 142301
%doi:10.1103/PhysRevLett.127.142301
[arXiv:2103.10403 [hep-ph]].
%159 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Becattini:2021suc}
\bibitem{Becattini:2021suc}
F.~Becattini, M.~Buzzegoli and A.~Palermo,
%``Spin-thermal shear coupling in a relativistic fluid,''
Phys. Lett. B \textbf{820} (2021), 136519
%doi:10.1016/j.physletb.2021.136519
[arXiv:2103.10917 [nucl-th]].
%133 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Becattini:2021iol}
\bibitem{Becattini:2021iol}
F.~Becattini, M.~Buzzegoli, G.~Inghirami, I.~Karpenko and A.~Palermo,
%``Local Polarization and Isothermal Local Equilibrium in Relativistic Heavy Ion Collisions,''
Phys. Rev. Lett. \textbf{127} (2021) no.27, 272302
%doi:10.1103/PhysRevLett.127.272302
[arXiv:2103.14621 [nucl-th]].
%160 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Florkowski:2019voj}
\bibitem{Florkowski:2019voj}
W.~Florkowski, A.~Kumar, R.~Ryblewski and A.~Mazeliauskas,
%``Longitudinal spin polarization in a thermal model,''
Phys. Rev. C \textbf{100} (2019) no.5, 054907
%doi:10.1103/PhysRevC.100.054907
[arXiv:1904.00002 [nucl-th]].
%88 citations counted in INSPIRE as of 23 Oct 2024

%\cite{Kapusta:2019sad}
\bibitem{Kapusta:2019sad}
J.~I.~Kapusta, E.~Rrapaj and S.~Rudaz,
%``Relaxation Time for Strange Quark Spin in Rotating Quark-Gluon Plasma,''
Phys. Rev. C \textbf{101} (2020) no.2, 024907
%doi:10.1103/PhysRevC.101.024907
[arXiv:1907.10750 [nucl-th]].
%37 citations counted in INSPIRE as of 22 Oct 2024

%\cite{Ayala:2020ndx}
\bibitem{Ayala:2020ndx}
A.~Ayala, D.~de la Cruz, L.~A.~Hern\'andez and J.~Salinas,
%``Relaxation time for the alignment between the spin of a finite-mass quark or antiquark and the thermal vorticity in relativistic heavy-ion collisions,''
Phys. Rev. D \textbf{102} (2020) no.5, 056019
%doi:10.1103/PhysRevD.102.056019
[arXiv:2003.06545 [hep-ph]].
%26 citations counted in INSPIRE as of 14 Nov 2024

%\cite{Kumar:2023ghs}
\bibitem{Kumar:2023ghs}
A.~Kumar, B.~M\"uller and D.~L.~Yang,
%``Spin alignment of vector mesons by glasma fields,''
Phys. Rev. D \textbf{108} (2023) no.1, 016020
%doi:10.1103/PhysRevD.108.016020
[arXiv:2304.04181 [nucl-th]].
%32 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Hidaka:2023oze}
\bibitem{Hidaka:2023oze}
Y.~Hidaka, M.~Hongo, M.~A.~Stephanov and H.~U.~Yee,
%``Spin relaxation rate for baryons in a thermal pion gas,''
Phys. Rev. C \textbf{109} (2024) no.5, 054909
%doi:10.1103/PhysRevC.109.054909
[arXiv:2312.08266 [hep-ph]].
%10 citations counted in INSPIRE as of 15 Nov 2024

%\cite{Wagner:2024fhf}
\bibitem{Wagner:2024fhf}
D.~Wagner, M.~Shokri and D.~H.~Rischke,
%``Damping of spin waves,''
Phys. Rev. Res. \textbf{6} (2024) no.4, 4
%doi:10.1103/PhysRevResearch.6.043103
[arXiv:2405.00533 [nucl-th]].
%13 citations counted in INSPIRE as of 14 Nov 2024

%\cite{Singh:2024cub}
\bibitem{Singh:2024cub}
S.~K.~Singh, R.~Ryblewski and W.~Florkowski,
%``Spin dynamics with realistic hydrodynamic background for relativistic heavy-ion collisions,''
[arXiv:2411.08223 [hep-ph]].
%0 citations counted in INSPIRE as of 15 Nov 2024

%%%%%%%% JAJATI NAYAK %%%%%


\bibitem{phot1} E. L. Feinberg, \ Nuovo \ Cim. {\bf A34}, 391 (1976).
\bibitem{phot2} G. David, \ Rept. \ Prog. \ Phys. {\bf 83}, 046301 (2020).
\bibitem{phot3} J. Alam, B. Sinha, and S. Raha, \ Phys. \ Rept.  {\bf 273}, 243 (1996).
\bibitem{phot4}  P. Stankus, \ Ann. \ Rev. \ Nucl. \ Part. \ Sci. {\bf 55}, 517 (2005).
\bibitem{kapustaprd} J. Kapusta, P. Lichard and D. Seibert {\it Phys. Rev. D} {\bf 44} (1991) 2774.
\bibitem{arnold2001}P. Arnold, G.D. Moore, and L.G. Yaffe, {\it J. High Energy Phys.} {\bf 0112} (2001) 009.
\bibitem{trg}S. Turbide, R. Rapp, and C. Gale, \ Phys. \ Rev. \ C   {\bf 69}, 014903 (2004).
\bibitem{nlo}J. Ghiglieri, J. Hong, A. Kurkela, E. Lu, G. D. Moore, D. Teaney,  JHEP  {\bf  05}, 010 (2013).
\bibitem{renk2003}T. Renk {\it Phys. Rev. C} {\bf 67}(2003) 064901.
\bibitem{jkn} J. K. Nayak and R. Chatterjee [in preparation].
\bibitem{pramana}R. Chatterjee, Pramana  {\bf 95}, 15 (2021).
\bibitem{fcc}P. Dasgupta, S. De, R. Chatterjee, D. K. Srivastava,  \ Phys. \ Rev. \ C  {\bf 98}, 02491 (2018).


%%%%%%%% Aswathy K Menon %%%%%%%%



\bibitem{CMS:2016fnw}
V.~Khachatryan \textit{et al.} [CMS Collaboration],
%``Evidence for collectivity in pp collisions at the LHC,''
Phys. Lett. B \textbf{765}, 193 (2017).

%\cite{Behera:2023nwj}
\bibitem{Behera:2023nwj}
D.~Behera, S.~Prasad, N.~Mallick and R.~Sahoo,
%``Effects of clustered nuclear geometry on the anisotropic flow in O-O collisions at the LHC within a multiphase transport model framework,''
Phys. Rev. D \textbf{108}, 054022 (2023).

%\cite{R:2024eni}
\bibitem{R:2024eni}
Aswathy~Menon~K.R., S.~Prasad, N.~Mallick and R.~Sahoo,
%``Role of clustered nuclear geometry in particle production through p--C and p--O collisions at the Large Hadron Collider,''
[arXiv:2407.03823 [nucl-th]] and the references therein.


%%%%%%% paramita deb %%%%%%%%


\bibitem{STAR} STAR Collaboration, J. Adams, and {\it et al.}, {\it Nucl. Phys. A} {\bf 757} (2005) 102.

\bibitem{rajagopal2000} B. Berdnikov and K. Rajagopal, {\it Phys. Rev. D} {\bf 61} (2000) 105017.

\bibitem{fukushima} K. Fukushima, {\it Phys. Lett. B} {\bf 591} (2004) 277.
\bibitem{ratti} C. Ratti, M. A. Thaler, and W. Weise, {\it Phys. Rev. D} {\bf 73} (2006) 014019.

\bibitem{deb2009} P. Deb, A. Bhattacharyya, S. Datta, and S. K. Ghosh, {\it Phys. Rev. C} {\bf 79} (2009) 055208.

\bibitem{deb2010a} A. Bhattacharyya, P. Deb, S. K. Ghosh, and R. Ray, {\it Phys. Rev. D} {\bf 82} (2010) 014021.

\bibitem{deb2010b} A. Bhattacharyya, P. Deb, A. Lahiri, and R. Ray, {\it Phys. Rev. D} {\bf 82} (2010) 114028.

\bibitem{deb2011} A. Bhattacharyya, P. Deb, A. Lahiri, and R. Ray, {\it Phys. Rev. D} {\bf 83} (2011) 014011.

\bibitem{deb2013} A. Bhattacharyya, P. Deb, S. K. Ghosh, R. Ray, and S. Sur, {\it Phys. Rev. D} {\bf 87} (2013) 054009.

\bibitem{nambu1961} Y. Nambu and G. Jona-Lasinio, {\it Physical Review} {\bf 122}, (1961) 345.

\bibitem{pisarski2000} A. Dumitru and R. D. Pisarski, {\it Phys. Lett. B} {\bf 525}, (2002) 95.

\bibitem{fukushima1} K. Fukushima, {\it Phys. Rev. D} {\bf 77}, (2008) 114028.

\bibitem{hansen2007} H. Hansen, W. M. Alberico, A. Beraudo, A. Molinari, M. Nardi, and C. Ratti, {\it Phys. Rev.D} {\bf 75}, (2007) 065004.

%\bibitem{deb2013} A. Bhattacharyya, P. Deb, S. K. Ghosh, R. Ray, and %S. Sur, {\it Phys. Rev. D} {\bf 87}, (2013) 054009.
%bloch1970,grunfeld2018

\bibitem{bloch1970} R. Balian and C. Bloch, {\it Annals of Physics} {\bf  60}, (1970) 401.

\bibitem{grunfeld2018} A. G. Grunfeld and G. Lugones, {\it The European Physical Journal C} {\bf 78}, (2018) 640.

\bibitem{karsch-strange2011} F. Karsch and K. Redlich, {\it Phys. Lett. B} {\bf 695}, (2011) 136.


\bibitem{STAR-proton2014} STAR Collaboration, L. Adamczyk, and et al., {\it Phys. Rev. Lett.} {\bf 113}, (2014) 092301.

\bibitem{STAR-charge2014} STAR Collaboration, L. Adamczyk, and et al., {\it Phys. Rev. Lett. 112}, (2014) 032302.

\bibitem{STAR-kaon2018} L. Adamczyk and et al., {\it Phys. Lett. B.} {\bf 785}, 551 (2018).


%%%%%%% pushpa %%%%%%%

\bibitem{gale} C. Gale, S. Jeon, and B. Schenke, \textit{Int. J. Mod. Phys. A} \textbf{28}, 1340011 (2013).

\bibitem{Heinz:2013th}
U.~Heinz and R.~Snellings,
%``Collective flow and viscosity in relativistic heavy-ion collisions,''
Ann. Rev. Nucl. Part. Sci. \textbf{63}, 123-151 (2013).
%doi:10.1146/annurev-nucl-102212-170540
%[arXiv:1301.2826 [nucl-th]].
%1369 citations counted in INSPIRE as of 28 Oct 2024

\bibitem{Jaiswal:2013vta}
A.~Jaiswal,
%``Relativistic third-order dissipative fluid dynamics from kinetic theory,''
\textit{Phys. Rev. C} \textbf{88}, 021903 (2013).
%doi:10.1103/PhysRevC.88.021903
%[arXiv:1305.3480 [nucl-th]].
%157 citations counted in INSPIRE as of 28 Oct 2024

\bibitem{Brito:2021iqr}
C.~V.~Brito and G.~S.~Denicol,
%``Linear causality and stability of third-order relativistic dissipative fluid dynamics,''
\textit{Phys. Rev. D} \textbf{105}, 096026 (2022).
%doi:10.1103/PhysRevD.105.096026
%[arXiv:2107.10319 [nucl-th]].
%20 citations counted in INSPIRE as of 28 Oct 2024

\bibitem{anderson}
J.~L.~ Anderson and H.~R.~Witting, \textit{Physica } \textbf{74}, 466-488 (1974).

\bibitem{Denicol:2010xn}
G.~S.~Denicol, T.~Koide and D.~H.~Rischke,
%``Dissipative relativistic fluid dynamics: a new way to derive the equations of motion from kinetic theory,''
\textit{Phys. Rev. Lett.} \textbf{105}, 162501 (2010).
%doi:10.1103/PhysRevLett.105.162501
%[arXiv:1004.5013 [nucl-th]].
%277 citations counted in INSPIRE as of 29 Oct 2024


%%%%%%% Sunny %%%%%%%

\bibitem{1} C. Gale, S. Jeon, and B. Schenke, {\it Int. J. Mod. Phys. A} {\bf 28} (2013) 1340011.

\bibitem{2} K. Tuchin, {\it Adv. High Energy Phys.} {\bf 2013} (2013) 490495.

\bibitem{3} K. Fukushima, D. E. Kharzeev, and H. J. Warringa, {\it Phys. Rev. D} {\bf 78} (2008) 074033.

\bibitem{4} D. Dash, S. Jaiswal, S. Bhadury, and A. Jaiswal, {\it Phys. Rev. C} {\bf 108} (2023) 064913.

\bibitem{5} S. Singh, M. Kurian, and V. Chandra, {\it Phys. Rev. D} {\bf 110} (2024) 014004.


\bibitem{6} Gabriel S. Rocha, Gabriel S. Denicol, and Jorge Noronha, {\it Phys. Rev. Lett} {\bf 127} (2021) 042301.

\bibitem{7} Gabriel S. Rocha, Caio V.P. de Brito, and Gabriel S. Denicol, {\it Phys. Rev. D} {\bf 108} (2021) 036017.


\bibitem{8} A. K. Panda, A. Dash, R. Biswas, and V. Roy, {\it JHEP} {\bf 03} (2021) 216.

%%%%%%% Victor %%%%%%%




%\cite{BRAHMS:2003wwg}
\bibitem{BRAHMS:2009wlg} I.~C.~Arsene \textit{et al.} [BRAHMS], 
{\it Phys. Lett. B} {\bf 677}, 267-271 (2009). 
doi:10.1016/j.physletb.2009.05.049 [arXiv:0901.0872 [nucl-ex]].

\bibitem{BRAHMS:2003wwg} I.~G.~Bearden \textit{et al.} [BRAHMS], 
{\it Phys. Rev. Lett.} {\bf 93}, 102301 (2004). 
doi:10.1103/PhysRevLett.93.102301 [arXiv:nucl-ex/0312023].

\bibitem{NA49:1998gaz} H.~Appelshauser \textit{et al.} [NA49], 
{\it Phys. Rev. Lett.} {\bf 82}, 2471-2475 (1999). 
doi:10.1103/PhysRevLett.82.2471 [arXiv:nucl-ex/9810014].




\bibitem{1} J. Callaway, {\it Phys. Rev. B} {\bf 35} (1987) 8723.

\bibitem{2} M. Lee, {\it Int. J. Phys.} {\bf 18}, 255 (2010) [Erratum: {\it ibid.} {\bf 18}, 440 (2010)].

\bibitem{3} M. Tinkham, {\it Group Theory and Quantum Mechanics}
(McGraw-Hill, New York, 1964).

\bibitem{4} T. Tel, in {\it Experimental Study and Characterization of
Chaos}, ed. B. Hao (World Scientific, Singapore, 1990),
p. 149.

\bibitem{Tong:lecturenotes} D.~Tong, 
{\it Lectures on Electromagnetism}. Available online: \url{www.damtp.cam.ac.uk/user/tong/em/el5.pdf}.


\bibitem{5}
P. P. Edwards, in {\it Superconductivity and Applications
--- Proc. Taiwan Int. Symp. on Superconductivity}, ed.  P. T. Wu
{\it et al.} (World Scientific, Singapore, 1989), p. 29.

\bibitem{6}
W. J. Johnson, Ph.D. Thesis, Univ. of Wisconsin, Madison (1968).

\bibitem{7}
P. F. Marteau and H. D. I. Arbabanel, ``Noise reduction in
chaotic time series using scaled probabilistic methods'',
UCSD/INLS preprint, October 1990.



%%%%%% sumit %%%%%%%



%\cite{McLerran:1984ay}
\bibitem{McLerran:1984ay}
L.~D.~McLerran and T.~Toimela,
%``Photon and Dilepton Emission from the Quark - Gluon Plasma: Some General Considerations,''
Phys. Rev. D \textbf{31} (1985), 545
%doi:10.1103/PhysRevD.31.545
%559 citations counted in INSPIRE as of 19 Dec 2022
				
%\cite{Linde:1980ts}
\bibitem{Linde:1980ts}
A.~D.~Linde,
%``Infrared Problem in Thermodynamics of the Yang-Mills Gas,''
Phys. Lett. B \textbf{96} (1980), 289-292
%doi:10.1016/0370-2693(80)90769-8
%835 citations counted in INSPIRE as of 19 Dec 2022

%\cite{Appelquist:1981vg}
\bibitem{Appelquist:1981vg}
T.~Appelquist and R.~D.~Pisarski,
%``High-Temperature Yang-Mills Theories and Three-Dimensional Quantum Chromodynamics,''
Phys. Rev. D \textbf{23} (1981), 2305
%doi:10.1103/PhysRevD.23.2305
%729 citations counted in INSPIRE as of 19 Dec 2022

				
%\cite{Detar:1987kae}
\bibitem{Detar:1987kae}
C.~E.~Detar and J.~B.~Kogut,
%``The Hadronic Spectrum of the Quark Plasma,''
Phys. Rev. Lett. \textbf{59} (1987), 399
%doi:10.1103/PhysRevLett.59.399
%203 citations counted in INSPIRE as of 19 Dec 2022	
	
%\cite{Laine:2003bd}
\bibitem{Laine:2003bd}
M.~Laine and M.~Vepsalainen,
%``Mesonic correlation lengths in high temperature QCD,''
JHEP \textbf{02} (2004), 004
%doi:10.1088/1126-6708/2004/02/004
%[arXiv:hep-ph/0311268 [hep-ph]].
%72 citations counted in INSPIRE as of 20 Dec 2022
	
%\cite{Bazavov:2019www}
\bibitem{Bazavov:2019www}
A.~Bazavov, 
%S.~Dentinger, H.~T.~Ding,P.~Hegde, O.~Kaczmarek, %F.~Karsch, E.~Laermann, A.~Lahiri, S.~Mukherjee and H.~Ohno, 
\textit{et al.}
%``Meson screening masses in (2+1)-flavor QCD,''
Phys. Rev. D \textbf{100} (2019) no.9, 094510
%doi:10.1103/PhysRevD.100.094510
%[arXiv:1908.09552 [hep-lat]].
%63 citations counted in INSPIRE as of 20 Dec 2022
	
%\cite{Gribov:1977wm}
\bibitem{Gribov:1977wm}
V.~N.~Gribov,
%``Quantization of Nonabelian Gauge Theories,''
Nucl. Phys. B \textbf{139} (1978), 1
%doi:10.1016/0550-3213(78)90175-X
%1829 citations counted in INSPIRE as of 20 Dec 2022	
	
%\cite{Sumit:2023hjj}
\bibitem{Sumit:2023hjj}
Sumit, N.~Haque and B.~K.~Patra,
%``QCD mesonic screening masses using Gribov quantization,''
Phys. Lett. B \textbf{845}, 138143 (2023)
%doi:10.1016/j.physletb.2023.138143
%[arXiv:2305.08525 [hep-ph]].
%6 citations counted in INSPIRE as of 30 Oct 2024	
	
%\cite{Fukushima:2013xsa}
\bibitem{Fukushima:2013xsa}
K.~Fukushima and N.~Su,
%``Stabilizing perturbative Yang-Mills thermodynamics with Gribov quantization,''
Phys. Rev. D \textbf{88} (2013), 076008
%doi:10.1103/PhysRevD.88.076008
%[arXiv:1304.8004 [hep-ph]].
%55 citations counted in INSPIRE as of 20 Dec 2022			
		
%\cite{Jaiswal:2020qmj}
\bibitem{Jaiswal:2020qmj}
A.~Jaiswal and N.~Haque,
%``Covariant kinetic theory and transport coefficients for Gribov plasma,''
Phys. Lett. B \textbf{811} (2020), 135936
%doi:10.1016/j.physletb.2020.135936
%[arXiv:2005.01303 [hep-ph]].
%5 citations counted in INSPIRE as of 20 Dec 2022




%%%%% rajkumar mondal %%%%%%%%%%

\bibitem{Tuchin:2013ie} Tuchin, Kirill {\it Adv. High Energy Phys.} {2013} (2013) 490495.

\bibitem{Kalikotay:2020snc} Kalikotay, Pallavi and Ghosh, Snigdha and Chaudhuri, Nilanjan and Roy, Pradip and Sarkar, Sourav {\it Phys. Rev. D} {102} (2020) 7, 076007.


\bibitem{Ozel:2016oaf} Ozel, Feryal and Freire, Paulo {\it Ann. Rev. Astron. Astrophys.} {54} (2016) 401--440.

\bibitem{Jaikumar:2021jbw} Jaikumar, Prashanth and Semposki, Alexandra and Prakash, Madappa and Constantinou, Constantinos {\it Phys. Rev. D} 103 (2021), 12, 123009.
		
	
\bibitem{Mondal:2023baz} Mondal, Rajkumar and Chaudhuri, Nilanjan and Roy, Pradip and Sarkar, Sourav, {\it Phys. Rev. C} {109} (2024) 054911.

\bibitem{Haber:2014ula} Haber, Alexander and Preis, Florian and Schmitt, Andreas {\it Phys. Rev. D} {90} (2014) 125036.

\bibitem{Ferrer:2010wz} Ferrer, Efrain J. and de la Incera, Vivian and Keith, Jason P. and Portillo, Israel and Springsteen, Paul L. {\it Phys. Rev. C} {82} (2010) 065802.

\bibitem{Ferrer:2022afu} Ferrer, E. J. and Hackebill, A. {\it Nucl. Phys. A} {1031} (2023) 122608



%%%%%%%%%% Rupa %%%%%%%%%%

\bibitem{fl1}
C. Adler \textit{et al.} (STAR Collaboration),
"Identified particle elliptic flow in Au + Au collisions at $\sqrt{s_{NN}} = 130$ GeV",
\textit{Phys. Rev. Lett.} \textbf{87}, 182301 (2001),
doi:10.1103/PhysRevLett.87.182301,
arXiv:nucl-ex/0107003.

\bibitem{fl4}
S. S. Adler \textit{et al.} (PHENIX Collaboration),
"Elliptic flow of identified hadrons in Au+Au collisions at $\sqrt{s_{NN}} = 200$ GeV",
\textit{Phys. Rev. Lett.} \textbf{91}, 182301 (2003),
doi:10.1103/PhysRevLett.91.182301,
arXiv:nucl-ex/0305013.

\bibitem{uli11}
U. Heinz, Z. Qiu, and C. Shen,
"Fluctuating flow angles and anisotropic flow measurements",
\textit{Phys. Rev. C} \textbf{87}, 034913 (2013),
doi:10.1103/PhysRevC.87.034913,
arXiv:1302.3535 [nucl-th].

\bibitem{hannu}
H. Holopainen, H. Niemi, and K. J. Eskola,
"Event-by-event hydrodynamics and elliptic flow from fluctuating initial state",
\textit{Phys. Rev. C} \textbf{83}, 034901 (2011),
doi:10.1103/PhysRevC.83.034901,
arXiv:1007.0368 [hep-ph].

\bibitem{qiu}
Z. Qiu, C. Shen, and U. Heinz,
"Hydrodynamic elliptic and triangular flow in Pb--Pb collisions at $\sqrt{s_{NN}} = 2.76$ A TeV",
\textit{Phys. Lett. B} \textbf{707}, 151--155 (2012),
doi:10.1016/j.physletb.2011.12.041.

\bibitem{gabor}
G. David,
"Direct real photons in relativistic heavy ion collisions",
\textit{Rept. Prog. Phys.} \textbf{83}, 046301 (2020),
doi:10.1088/1361-6633/ab6f57,
arXiv:1907.08893.

\bibitem{chun_prl}
C. Shen, J.-F. Paquet, G. S. Denicol, S. Jeon, and C. Gale,
"Thermal photon radiation in high multiplicity p+Pb collisions at the Large Hadron Collider",
\textit{Phys. Rev. Lett.} \textbf{116}, 072301 (2016),
doi:10.1103/PhysRevLett.116.072301,
arXiv:1504.07989 [nucl-th].

\bibitem{phot11}
J. Alam, B. Sinha, and S. Raha,
"Electromagnetic probes of quark gluon plasma",
\textit{Phys. Rept.} \textbf{273}, 243--362 (1996),
doi:10.1016/0370-1573(95)00084-4.

\bibitem{phot2}
W. Cassing and E. L. Bratkovskaya,
"Hadronic and electromagnetic probes of hot and dense nuclear matter",
\textit{Phys. Rept.} \textbf{308}, 65--233 (1999),
doi:10.1016/S0370-1573(98)00028-3.

\bibitem{phot3}
T. Peitzmann and M. H. Thoma,
"Direct photons from relativistic heavy ion collisions",
\textit{Phys. Rept.} \textbf{364}, 175--246 (2002),
doi:10.1016/S0370-1573(02)00012-1,
arXiv:hep-ph/0111114.

\bibitem{phot4}
P. Stankus,
"Direct photon production in relativistic heavy-ion collisions",
\textit{Ann. Rev. Nucl. Part. Sci.} \textbf{55}, 517--554 (2005),
doi:10.1146/annurev.nucl.53.041002.110533.

\bibitem{phot6}
C. Shen, U. W. Heinz, J.-F. Paquet, and C. Gale,
"Thermal photons as a quark-gluon plasma thermometer reexamined",
\textit{Phys. Rev. C} \textbf{89}, 044910 (2014),
doi:10.1103/PhysRevC.89.044910,
arXiv:1308.2440 [nucl-th].

\bibitem{phot7}
J.-F. Paquet,
"Probing the space-time evolution of heavy ion collisions with photons and dileptons",
\textit{Nucl. Phys. A} \textbf{967}, 184--191 (2017),
doi:10.1016/j.nuclphysa.2017.06.003,
arXiv:1704.07842 [nucl-th].

\bibitem{phot8}
Gale, Charles. "Direct photon production in relativistic heavy-ion collisions - a theory update." *PoS*, High-pT2017 (2019): 023. arXiv:1802.00128 [hep-ph]. doi:10.22323/1.320.0023.

\bibitem{phot}
McLerran, Larry D. and Toimela, T. "Photon and Dilepton Emission from the Quark - Gluon Plasma: Some General Considerations." *Phys. Rev. D* 31 (1985): 545. doi:10.1103/PhysRevD.31.545.

\bibitem{dks}
Srivastava, Dinesh K. "Direct photons from relativistic heavy-ion collisions." In *J. Phys. G* 35, no. 10 (2008): 104026. arXiv:0805.3401 [nucl-th]. doi:10.1088/0954-3899/35/10/104026.

\bibitem{emprobes}
Chatterjee, Rupa, Bhattacharya, Lusaka, and Srivastava, Dinesh K. "Electromagnetic probes." In *Lect. Notes Phys.* 785 (2010): 219–264. arXiv:0901.3610 [nucl-th]. doi:10.1007/978-3-642-02286-97.

\bibitem{rc_pramana}
Chatterjee, Rupa. "Anisotropic flow of photons in relativistic heavy ion collisions." *Pramana* 95, no. 1 (2021): 15. doi:10.1007/s12043-020-02038-0.

\bibitem{Gale:2014dfa}
Gale, Charles, et al. "Production and Elliptic Flow of Dileptons and Photons in a Matrix Model of the Quark-Gluon Plasma." *Phys. Rev. Lett.* 114 (2015): 072301. arXiv:1409.4778 [hep-ph]. doi:10.1103/PhysRevLett.114.072301.

\bibitem{Monnai}
Monnai, Akihiko. "Thermal photon $v_2$ with slow quark chemical equilibration." *Phys. Rev. C* 90, no. 2 (2014): 021901. arXiv:1403.4225 [nucl-th]. doi:10.1103/PhysRevC.90.021901.

\bibitem{Vujanovic}
Vujanovic, Gojko, et al. "Probing the early-time dynamics of relativistic heavy-ion collisions with electromagnetic radiation." *Nucl. Phys. A* 932 (2014): 230–234. arXiv:1404.3714 [hep-ph]. doi:10.1016/j.nuclphysa.2014.08.053.

\bibitem{Liu:2012ax}
Liu, Fu-Ming, and Liu, Sheng-Xu. "Quark-gluon plasma formation time and direct photons from heavy ion collisions." *Phys. Rev. C* 89, no. 3 (2014): 034906. doi:10.1103/PhysRevC.89.034906.

\bibitem{oscar}
Garcia-Montero, Oscar, et al. "Probing the evolution of heavy-ion collisions using direct photon interferometry." *Phys. Rev. C* 102, no. 2 (2020): 024915. doi:10.1103/PhysRevC.102.024915.

\bibitem{phot1}
Ruuskanen, P.V. "Electromagnetic probes of quark-gluon plasma in relativistic heavy-ion collisions." *Nuclear Physics A* 544, no. 1 (1992): 169–182. doi:10.1016/0375-9474(92)90572-2.

\bibitem{i1}
Srivastava, Dinesh K., and Kapusta, Joseph I. "Photon interferometry of quark-gluon dynamics." *Phys. Lett. B* 307, no. 1 (1993): 1–6. doi:10.1016/0370-2693(93)90183-I.

\bibitem{i2}
Srivastava, Dinesh Kumar. "Intensity interferometry of thermal photons from relativistic heavy ion collisions." *Phys. Rev. C* 71 (2005): 034905. arXiv:nucl-th/0411041. doi:10.1103/PhysRevC.71.034905.

\bibitem{i3}
Peressounko, D. "Hanbury Brown-Twiss interferometry of direct photons in heavy ion collisions." *Phys. Rev. C* 67 (2003): 014905. doi:10.1103/PhysRevC.67.014905.

\bibitem{i4}
Frodermann, Evan, and Heinz, Ulrich. "Photon HBT interferometry for non-central heavy-ion collisions." *Phys. Rev. C* 80 (2009): 044903. arXiv:0907.1292 [nucl-th]. doi:10.1103/PhysRevC.80.044903.

\bibitem{rhic}
Adare, A., et al. "Centrality dependence of low-momentum direct-photon production in Au$+$Au collisions at $\sqrt{s_{_{NN}}}=200$ GeV." *Phys. Rev. C* 91, no. 6 (2015): 064904. arXiv:1405.3940 [nucl-ex]. doi:10.1103/PhysRevC.91.064904.

\bibitem{lhc}
Adam, Jaroslav, et al. "Direct photon production in Pb-Pb collisions at $\sqrt{s_{NN}} =$ 2.76 TeV." *Phys. Lett. B* 754 (2016): 235–248. arXiv:1509.07324 [nucl-ex]. doi:10.1016/j.physletb.2016.01.020.

\bibitem{hardprobes}
Chatterjee, Rupa. "Electroweak Physics: Summary." *PoS*, HardProbes2020 (2021): 026. arXiv:2106.12922 [nucl-th]. doi:10.22323/1.387.0026.

\bibitem{phe1}
Adare, A., et al. "Low-momentum direct photon measurement in Cu$+$Cu collisions at $\sqrt{s_{_{NN}}}=200$ GeV." *Phys. Rev. C* 98, no. 5 (2018): 054902. arXiv:1805.04066 [hep-ex]. doi:10.1103/PhysRevC.98.054902.

\bibitem{phe2}
Adare, A. et al. (PHENIX Collaboration), 
"Beam Energy and Centrality Dependence of Direct-Photon Emission from Ultrarelativistic Heavy-Ion Collisions," 
\textit{Phys. Rev. Lett.} \textbf{123}, 022301 (2019). 
DOI: 10.1103/PhysRevLett.123.022301. 
arXiv:1805.04084.

\bibitem{cfhs}
Chatterjee, R., Frodermann, E. S., Heinz, U. W., and Srivastava, D. K., 
"Elliptic flow of thermal photons in relativistic nuclear collisions," 
\textit{Phys. Rev. Lett.} \textbf{96}, 202302 (2006). 
DOI: 10.1103/PhysRevLett.96.202302. 
arXiv:nucl-th/0511079.

\bibitem{rc_tau0}
Chatterjee, R. and Srivastava, D. K., 
"Formation Time of QGP from Thermal Photon Elliptic Flow," 
\textit{Nucl. Phys. A} \textbf{830}, 503C–506C (2009). 
DOI: 10.1016/j.nuclphysa.2009.10.043. 
arXiv:0907.3548.

\bibitem{rc_dil}
Chatterjee, R., Srivastava, D. K., Heinz, U. W., and Gale, C., 
"Elliptic flow of thermal dileptons in relativistic nuclear collisions," 
\textit{Phys. Rev. C} \textbf{75}, 054909 (2007). 
DOI: 10.1103/PhysRevC.75.054909. 
arXiv:nucl-th/0702039.

\bibitem{rc_v3}
Chatterjee, R., Srivastava, D. K., and Renk, T., 
"Triangular flow of thermal photons from an event-by-event hydrodynamic model for 2.76A TeV Pb + Pb collisions at the CERN Large Hadron Collider," 
\textit{Phys. Rev. C} \textbf{94}, 014903 (2016). 
DOI: 10.1103/PhysRevC.94.014903. 
arXiv:1401.7464.

\bibitem{viscometer}
Shen, C., Heinz, U., Paquet, J.-F., and Gale, C., 
"Thermal photon anisotropic flow serves as a quark-gluon plasma viscometer," 
\textit{Nucl. Phys. A} \textbf{932}, 184 (2014). 
DOI: 10.1016/j.nuclphysa.2014.07.042. 
arXiv:1403.7558.

\bibitem{v2_v3}
Chatterjee, R., Dasgupta, P., and Srivastava, D. K., 
"Anisotropic flow of thermal photons at energies available at the BNL Relativistic Heavy Ion Collider and at the CERN Large Hadron Collider," 
\textit{Phys. Rev. C} \textbf{96}, 014911 (2017). 
DOI: 10.1103/PhysRevC.96.014911. 
arXiv:1702.02378.

\bibitem{phenix_phot}
Adare, A. et al. (PHENIX Collaboration), 
"Azimuthally anisotropic emission of low-momentum direct photons in Au$+$Au collisions at $\sqrt{s_{NN}}=200$ GeV," 
\textit{Phys. Rev. C} \textbf{94}, 064901 (2016). 
DOI: 10.1103/PhysRevC.94.064901. 
arXiv:1509.07758.

\bibitem{p1}
Adare, A. et al. (PHENIX Collaboration), 
"Observation of direct-photon collective flow in $\sqrt{s_{NN}}=200$ GeV Au+Au collisions," 
\textit{Phys. Rev. Lett.} \textbf{109}, 122302 (2012). 
DOI: 10.1103/PhysRevLett.109.122302. 
arXiv:1105.4126.

\bibitem{l1}
Lohner, D. (ALICE Collaboration), 
"Measurement of Direct-Photon Elliptic Flow in Pb-Pb Collisions at $\sqrt{s_{NN}} = 2.76$ TeV," 
\textit{J. Phys. Conf. Ser.} \textbf{446}, 012028 (2013). 
DOI: 10.1088/1742-6596/446/1/012028. 
arXiv:1212.3995.

\bibitem{rc_phot_fluc}
Chatterjee, R., Holopainen, H., Renk, T., and Eskola, K. J., 
"Enhancement of thermal photon production in event-by-event hydrodynamics," 
\textit{Phys. Rev. C} \textbf{83}, 054908 (2011). 
DOI: 10.1103/PhysRevC.83.054908. 
arXiv:1102.4706.

\bibitem{rc_v2_fluc}
Chatterjee, R., Holopainen, H., Helenius, I., Renk, T., and Eskola, K. J., 
"Elliptic flow of thermal photons from event-by-event hydrodynamic model," 
\textit{Phys. Rev. C} \textbf{88}, 034901 (2013). 
DOI: 10.1103/PhysRevC.88.034901. 
arXiv:1305.6443.

\bibitem{v2_1}
van Hees, H., Gale, C., and Rapp, R., 
"Thermal Photons and Collective Flow at the Relativistic Heavy-Ion Collider," 
\textit{Phys. Rev. C} \textbf{84}, 054906 (2011). 
DOI: 10.1103/PhysRevC.84.054906. 
arXiv:1108.2131.

\bibitem{v2_2}
Linnyk, O., Cassing, W., and Bratkovskaya, E. L., 
"Centrality dependence of the direct photon yield and elliptic flow in heavy-ion collisions at $\sqrt{s_{NN}}=200$ GeV," 
\textit{Phys. Rev. C} \textbf{89}, 034908 (2014). 
DOI: 10.1103/PhysRevC.89.034908. 
arXiv:1311.0279.

\bibitem{v2_3}
Gale, C., Hidaka, Y., Jeon, S., Lin, S., Paquet, J.-F., Pisarski, R. D., Satow, D., Skokov, V. V., and Vujanovic, G., 
"Production and Elliptic Flow of Dileptons and Photons in a Matrix Model of the Quark-Gluon Plasma," 
\textit{Phys. Rev. Lett.} \textbf{114}, 072301 (2015). 
DOI: 10.1103/PhysRevLett.114.072301. 
arXiv:1409.4778.

\bibitem{v2_4}
Basar, G., Kharzeev, D., and Skokov, V., 
"Conformal anomaly as a source of soft photons in heavy ion collisions," 
\textit{Phys. Rev. Lett.} \textbf{109}, 202303 (2012). 
DOI: 10.1103/PhysRevLett.109.202303. 
arXiv:1206.1334.

\bibitem{v1}
Dasgupta, P., Chatterjee, R., and Srivastava, D. K., 
"Directed flow of photons in Cu+Au collisions at RHIC," 
\textit{J. Phys. G} \textbf{47}, 085101 (2020). 
DOI: 10.1088/1361-6471/ab920e. 
arXiv:1901.04943.

\bibitem{fcc}
Dasgupta, P., De, S., Chatterjee, R., and Srivastava, D. K., 
"Photon production from Pb+Pb collisions at $\sqrt{s_{\rm {NN}}}$ = 5.02 TeV at LHC and at $\sqrt{s_{\rm {NN}}}$ = 39 TeV at FCC," 
\textit{Phys. Rev. C} \textbf{98}, 024911 (2018). 
DOI: 10.1103/PhysRevC.98.024911. 
arXiv:1804.02828.


\bibitem{a1} 
C.~Gale, Y.~Hidaka, S.~Jeon, S.~Lin, J.~F.~Paquet, R.~D.~Pisarski, D.~Satow, V.~V.~Skokov, and G.~Vujanovic, 
``Production and Elliptic Flow of Dileptons and Photons in a Matrix Model of the Quark-Gluon Plasma,'' 
\emph{Phys. Rev. Lett.} \textbf{114}, 072301 (2015). 
DOI: 10.1103/PhysRevLett.114.072301.

\bibitem{a2}
A.~Monnai, 
``Thermal photon $v_2$ with slow quark chemical equilibration,'' 
\emph{Phys. Rev. C} \textbf{90}, 021901 (2014). 
DOI: 10.1103/PhysRevC.90.021901.

\bibitem{rc_fluc_tau0} 
R.~Chatterjee, H.~Holopainen, T.~Renk, and K.~J.~Eskola, 
``Collision centrality and $\tau_0$ dependence of the emission of thermal photons from fluctuating initial state in ideal hydrodynamic calculation,'' 
\emph{Phys. Rev. C} \textbf{85}, 064910 (2012). 
DOI: 10.1103/PhysRevC.85.064910.

\bibitem{ratio}
R.~Chatterjee and P.~Dasgupta, 
``Ratio of photon anisotropic flow in relativistic heavy ion collisions,'' 
\emph{Phys. Rev. C} \textbf{104}, 064907 (2021). 
DOI: 10.1103/PhysRevC.104.064907.

\bibitem{small1}
C.~Aidala \emph{et al.} [PHENIX Collaboration], 
``Creation of quark-gluon plasma droplets with three distinct geometries,'' 
\emph{Nature Phys.} \textbf{15}, 214-220 (2019). 
DOI: 10.1038/s41567-018-0360-0.

\bibitem{sanchari} 
S.~Thakur, P.~Dasgupta, S.~Prasad, and R.~Chatterjee, 
``Study of initial state on O+O collisions at 7 TeV,'' 
68th DAE BRNS Symposium on Nuclear Physics, 2024.

\bibitem{small2}
G.~Aad \emph{et al.} [ATLAS Collaboration], 
``Observation of Long-Range Elliptic Azimuthal Anisotropies in $\sqrt{s}=$13 and 2.76 TeV $pp$ Collisions with the ATLAS Detector,'' 
\emph{Phys. Rev. Lett.} \textbf{116}, 172301 (2016). 
DOI: 10.1103/PhysRevLett.116.172301.

\bibitem{small3}
S.~Chatrchyan \emph{et al.} [CMS Collaboration], 
``Observation of Long-Range Near-Side Angular Correlations in Proton-Lead Collisions at the LHC,'' 
\emph{Phys. Lett. B} \textbf{718}, 795-814 (2013). 
DOI: 10.1016/j.physletb.2012.11.025.

\bibitem{c1}
M.~Rybczyński, M.~Piotrowska, and W.~Broniowski, 
``Signatures of $\alpha$ clustering in ultrarelativistic collisions with light nuclei,'' 
\emph{Phys. Rev. C} \textbf{97}, 034912 (2018). 
DOI: 10.1103/PhysRevC.97.034912.

\bibitem{c2}
P.~Bozek, W.~Broniowski, E.~Ruiz Arriola, and M.~Rybczynski, 
``$\alpha$ clusters and collective flow in ultrarelativistic carbon-heavy-nucleus collisions,'' 
\emph{Phys. Rev. C} \textbf{90}, 064902 (2014). 
DOI: 10.1103/PhysRevC.90.064902.

\bibitem{c3}
D.~Behera, S.~Deb, C.~R.~Singh, and R.~Sahoo, 
``Characterizing nuclear modification effects in high-energy O-O collisions at energies available at the CERN Large Hadron Collider: A transport model perspective,'' 
\emph{Phys. Rev. C} \textbf{109}, 014902 (2024). 
DOI: 10.1103/PhysRevC.109.014902.

\bibitem{rc_cluster}
P.~Dasgupta, G.~L.~Ma, R.~Chatterjee, L.~Yan, S.~Zhang, and Y.~G.~Ma, 
``Thermal photons as a sensitive probe of $\alpha$-cluster in C + Au collisions at the BNL Relativistic Heavy Ion Collider,'' 
\emph{Eur. Phys. J. A} \textbf{57}, 134 (2021). 
DOI: 10.1140/epja/s10050-021-00441-8.

\bibitem{cluster_ebye}
P.~Dasgupta, R.~Chatterjee, and G.~L.~Ma, 
``Production and anisotropic flow of thermal photons in collisions of $\alpha$-clustered carbon with heavy nuclei at relativistic energies,'' 
\emph{Phys. Rev. C} \textbf{107}, 044908 (2023). 
DOI: 10.1103/PhysRevC.107.044908.




